Quantum Bisimilarity is a Congruence under Physically Admissible Schedulers

The development of quantum algorithms and protocols calls for adequate modelling and verification techniques, which requires abstracting and focusing on the basic features of quantum concurrent systems, like CCS and CSP have done for their classical counterparts. So far, an equivalence relation is still missing that is a congruence for parallel composition and adheres to the limited discriminating power implied by quantum theory. In fact, defining an adequate bisimilarity for quantum-capable, concurrent systems proved a difficult task, because unconstrained non-determinism allows to spuriously discriminate indistinguishable quantum systems. We investigate this problem by enriching a linear quantum extension of CCS with simple physically admissible schedulers. We show that our approach suffices for deriving a well-behaved bisimilarity that satisfies the aforementioned desiderata.

==> Sections/better.tex <==
\red{
\textbf{Esempio con rose che non dovrebbero essere bisimili, ma riducono agli stessi processi o distribuzioni.}}

==> Sections/lemma_backwards.tex <==

\begin{lemma}\label{interpretbw} %
	For any observer $R$ and index $\lambda \neq \diamond$, we have
	\[\forall k \ \left( \conf{\rho, P \parallel \ptag{R}_k}  \rightarrow \Delta : k\lambda
	\Longrightarrow	
	\conf{\rho, P, R} \longsquiggly_\lambda \Delta' \text{ with } \ptag{\Delta'}_k^{\lambda} \equiv \Delta
	\right)\]
\end{lemma}
\begin{proof}

Note that any transition $\ptag{\mathcal{C}}_k = \conf{\rho, P \parallel \ptag{R}_k}  \rightarrow \Delta : k\lambda$ must involve $R$, because a transition modifying only $P$ would not be tagged as $k\lambda$. We will then proceed on induction on the syntax of $R$.

If $R = \nil_{\tilde{e}}$, there are no $k\lambda$-tagged transitions going out from $\ptag{\conf{\rho, P\parallel \nil_{\tilde{e}}}} =  \conf{\rho, P\parallel \nil_{\tilde{e}}}$.

If $R = \sop{E}{\tilde{x}}.R' $, we have \[\ptag{\mathcal{C}}_k \equiv \conf{\rho, P \parallel \sop{E}{\tilde{x}}.\ptag{R'}_{k\barr} + k!0} \rightarrow \Delta \equiv \singleton{\conf{\sop[\tilde{e}]{E}{\rho}, P \parallel \ptag{R'}_{k\barr}}}~:~k\]
But then 
\begin{align*}
&\conf{\rho, P, \sop{E}{\tilde{x}}.R'} \longsquiggly_\varepsilon \Delta' = \singleton{\conf{\sop[\tilde{e}]{E}{\rho}, P, R'}}, \text{ and }\\
&\ptag{\Delta'}_k^{\varepsilon} = \singleton{\conf{\sop[\tilde{e}]{E}{\rho}, P \parallel \ptag{R'}_{k}^{\varepsilon}}} = \singleton{\conf{\sop[\tilde{e}]{E}{\rho}, P \parallel \ptag{R'}_{k\barr}}} \equiv \Delta.
\end{align*}

If $R = \meas{\tilde{x}}{y}.R'$, we have
\[\conf{\rho, P \parallel \meas{\tilde{x}}{y}.\ptag{R'}_{k\barr} + \varepsilon!0} \rightarrow \Delta \equiv \sum_m \distelem{p_m}{\singleton{\conf{\rho_m, P \parallel \ptag{R'}_{k\barr}[m/y]}}} : \varepsilon\]
for some set of $p_m$ and $\rho_m$. Then the proof is identical to the previous case, noticing that $\ptag{R[v/x]}_k^\lambda = \ptag{R}_k^\lambda[v/x]$ as the tags depends on the position of the processes and not on their content.

If $R = c!e $, then $P$ must be receiving on the unrestricted channel $c$, so we have \[\ptag{\mathcal{C}}_k \equiv \conf{\rho, (((c?x.P') + P'') \parallel Q \parallel (c!v + \varepsilon!0)) \setminus D} \rightarrow \Delta \equiv \singleton{\conf{\rho, ( P'[v/x] \parallel Q )\setminus D}}~:~\varepsilon\]
for some (possibly empty) set of restrictions $D$ and processes $P', P'', Q$. But then \\ $\mathcal{C} \equiv_o \conf{\rho, (((c?x.P') + P'') \parallel Q)  \setminus D, c!v} \longsquiggly_\varepsilon \Delta' = \singleton{\conf{\rho, ( P'[v/x] \parallel Q )\setminus D, \nil}}$ and $\ptag{\Delta'}_k^{\varepsilon} \equiv \Delta$.

If $R$ is a sum of reception, then $P$ must be sending on at least one of the channel in $R$, so we have 
\[\ptag{\mathcal{C}}_k \equiv \conf{\rho, (((c!v + P) \parallel Q \parallel (c?x.\ptag{R'}_{k\barr} + \ptag{T}_k + \varepsilon!0)) \setminus D} \rightarrow \Delta \equiv \singleton{\conf{\rho, ( Q \setminus D )\parallel R'[v/x]}}~:~\varepsilon\]
for some (possibly empty) set of restrictions $D$ and process $Q$, and the proof is identical to the previous case.

If $R = \ite{e}{R_1}{R_2}$, then the only way to have a transition is after applying the structural congruence and obtaining either $R_1$ or $R_2$, from which the desired property is obtained thanks to the inductive hypothesis and the fact that $\ptag{R}_k \equiv \ptag{R'}_k$ if and only if $R \equiv_o R'$.

If $R =  R_1 \expar R_2 $ and $\ptag{\mathcal{C}}_k \equiv \conf{\rho, P \parallel \ptag{R_1}_{kl} \parallel \ptag{R_2}_{kr}} \rightarrow \Delta : k\lambda$, then the transition cannot be a synchronisation between $R_1$ and $R_2$ because all the tags of $\ptag{C}_k$ must be in $\Delta$ except from $k\lambda$, and a synchronisation would destroy two tags, not just one. Suppose then that the transition involves $R_1$, the $R_2$ case is symmetric. From the $\rulename{SemPar}$ rule must be $\conf{\rho, P \parallel \ptag{R_1}_{k\ell}} \rightarrow \Delta_\ell$ with $\Delta = \Delta_\ell \parallel\ptag{R_2}_{kr} $.  This transition is still tagged with $k\lambda$, as the $k\lambda$ tag is present in $\ptag{R_1}_{k\ell} \parallel \ptag{R_2}_{kr}$ but is absent in $\Delta_\ell \parallel\ptag{R_2}_{kr}$, no must be in $\ptag{R_1}_{kl}$. Besides, we know that $k\lambda = k\ell\lambda'$ for some $\lambda'$, as it is easy to verify that all the tags in $\ptag{R_1}_{k\ell}$ start with $k\ell$. Then we can apply the inductive hypothesis 
\begin{gather*}
\conf{\rho, P \parallel \ptag{R_1}_{k\ell}} \rightarrow \Delta_\ell :k\ell\lambda' 
\qquad \Rightarrow  \qquad
\conf{\rho, P, R_1} \longsquiggly_{\lambda'} \Delta_\ell' \text{ with } \ptag{\Delta_\ell'}_{k\ell}^{\lambda'} = \Delta_\ell
\end{gather*}
and derive 
\[\conf{\rho, P, R_1 \expar R_2} \longsquiggly_{\lambda} \Delta' = \Delta_\ell'\parallel R_2 \text{ with } \ptag{\Delta'}_k^{\lambda} = \Delta
\]
since $\lambda = \ell\lambda'$ and $\ptag{\Delta'}_k^{\lambda} = \ptag{\Delta_\ell'\parallel R_2}_k^{\ell\lambda'} = \ptag{\Delta_\ell'}_{k\ell}^{\lambda'} \parallel \ptag{R_2}_{kr}  = \Delta_\ell \parallel \ptag{R_2}_{kr} = \Delta$.
\end{proof}





==> Sections/lemma_forward.tex <==

\begin{lemma}\label{interpretfw} %
  For any observer $R$ and index $\lambda \neq \diamond$, we have
  \[
    \forall k \ldotp \conf{\rho, P, R} \longsquiggly_\lambda \Delta \Longrightarrow
    \conf{\rho, P \parallel \ptag{R}_k} \to \ptag{\Delta}^\lambda_k : k\lambda
  \]
\end{lemma}
\begin{proof}
  We will proceed by induction on the transition $\longsquiggly_\lambda$.

  If rule \textsc{OQOp} is valid, then $R \equiv \sop{E}{\tilde{q}}.R_1$, we
  have
  \[
    \iconf = \conf{\rho, P, \sop{E}{\tilde{q}}.R_1} \longsquiggly_\varepsilon
    \sconf{\mathcal{E}_{\tilde{q}}(\rho), P, R_1} = \Delta
  \]
  and
  \[
    \ptag{\iconf}_k =
    \conf{\rho, P \parallel (\sop{E}{\tilde{q}}.\ptag{R_1}_{k\barr} +
    k!0)}
    \to \sconf{\mathcal{E}_{\tilde{q}}(\rho), P \parallel \ptag{R_1}_{k\barr}} =
    \ptag{\Delta}^\varepsilon_k
  \]
  We must further check that:
  $\ptag{\iconf}_k \to \ptag{\Delta}^\varepsilon_k :
  k$. The first condition, $k \in T(\ptag{\iconf}_k)$, is true by $k!0$.
  The second, $k \not\in T(\iconf')$, is true because any new barb expressed by $\ptag{R_1}_{k\barr}$ must start with
  $k\barr$. The third condition, $T(\ptag{\iconf}_k) \setminus \{k\} \subseteq
  T(\ptag{\Delta}^\varepsilon_k)$, is also trivially true since the only syntactic difference between the $\iconf$ and
  $\Delta$ is the barb-expressing $k!0$.

  If rule \textsc{OQMeas} is valid, then $R \equiv \meas{\tilde{q}}{y}.R_1$, we
  have
  \[
    \iconf = \conf{\rho, P, \meas{\tilde{q}}{y}.R_1} \longsquiggly_\varepsilon
    \sum_{i=0}^{|M| - 1}\distelem{p_m}{\sconf{\frac{\rho_m}{p_m}, P, R_1[\sfrac{m}{y}]}} = \Delta
  \]
  and, noting as before that $\ptag{R[\sfrac{v}{x}]}^\lambda_k =
  \ptag{R}^\lambda_k[\sfrac{v}{x}]$
  \[
    \ptag{\iconf}_k
    = \conf{\rho, P \parallel (\meas{\tilde{q}}{y}.\ptag{R_1}_{k\barr} +
    k!0)}
    \to \sum_{i=0}^{|M| - 1}\distelem{p_m}{\sconf{\frac{\rho_m}{p_m}, P \parallel
    (\ptag{R_1}_{k\barr}[\sfrac{m}{y}] + k!0)}} =
    \ptag{\Delta}^\varepsilon_k
  \]
  $\ptag{\iconf}_k \to \ptag{\Delta}^\varepsilon_k :
  k$ holds as for the \textsc{OQOp} noting that each element in
  $\ptag{\Delta}^\varepsilon_k$ has syntactically the same sendings.

  If rule \textsc{Input} is valid, then $R \equiv c?x.R_1 + R_2$, we have
  \[
    \iconf =
    \conf{\rho, (c!v + P_1) \parallel P_2 \setminus D, c?x.R_1 + R_2} 
    \longsquiggly_\varepsilon \sconf{\rho, P_2 \setminus D, R_1[\sfrac{v}{x}]}
    = \Delta
  \]
  and
  \begin{align*}
    \ptag{\iconf}_k
    &= \conf{\rho, ((c!v + P_1) \parallel P_2 \setminus D) \parallel (c?x.\ptag{R_1}_{k\barr} + k!0 + \ptag{R_2}_k)} \\
    &\equiv \conf{\rho, ((c!v + P_1) \parallel P_2 \parallel (c?x.\ptag{R_1}_{k\barr} + k!0 + \ptag{R_2}_k)) \setminus D} \\
    &\to \sconf{\rho, (P_2 \parallel \ptag{R_1}_{k\barr}[\sfrac{v}{x}]) \setminus D} \\
    &\equiv \sconf{\rho, (P_2 \setminus D) \parallel \ptag{R_1[\sfrac{v}{x}]}_{k\barr}}
    = \ptag{\Delta}^\varepsilon_k
  \end{align*}
  $\ptag{\iconf}_k \to \ptag{\Delta}^\varepsilon_k :
  k$ holds trivially as for the \textsc{OQOp}.

  If rule \textsc{Output} is valid, then $R \equiv c!v$, we have
  \[
    \iconf =
    \conf{\rho, (c?x.P_1) + P_2) \parallel P_3 \setminus D, c!v} 
    \longsquiggly_\varepsilon \sconf{\rho, (P_1[\sfrac{v}{x}] \parallel P_3) \setminus D, \nil}
    = \Delta
  \]
  and
  \begin{align*}
    \ptag{\iconf}_k
    &= \conf{\rho, (((c?x.P_1) + P_2) \parallel P_3 \setminus D) \parallel (c!v + k!0)} \\
    &\equiv \conf{\rho, (((c?x.P_1) + P_2) \parallel P_3 \parallel (c!v + k!0)) \setminus D} \\
    &\to \sconf{\rho, (P_1[\sfrac{v}{x}] \parallel P_3 \parallel \nil) \setminus D} \\
    &\equiv \sconf{\rho, (P_1[\sfrac{v}{x}] \parallel P_3 \setminus D) \parallel \nil}
    = \ptag{\Delta}^\varepsilon_k
  \end{align*}
  $\ptag{\iconf}_k \to \ptag{\Delta}^\varepsilon_k :
  k$ holds trivially as for the \textsc{QInput}.

  If rule \textsc{ParL} is valid, then $R \equiv R_1 \parallel R_2$, we have
  \[
    \iconf =
    \conf{\rho, P, R_1 \parallel R_2}
    \longsquiggly_{\ell\lambda} \Theta \parallel R_2
    = \Delta
  \]
  By inductive hypothesis, for any $k$
  \[
    \conf{\rho, P, R_1} \longsquiggly_\lambda \Theta \Longrightarrow \conf{\rho, P \parallel \ptag{R_1}_k} \to \ptag{\Theta}^\lambda_k : k\lambda
  \]
  and
  \begin{align*}
    \ptag{\iconf}_k
    = \conf{\rho, P \parallel \ptag{R_1}_{k\ell} \parallel \ptag{R_2}_{kr}}
    \to \ptag{\Theta}^\lambda_{k\ell} \parallel \ptag{R_2}_{kr}
    = \ptag{\Delta}^{\ell\lambda}_k
  \end{align*}
  $\ptag{\iconf}_k \to \ptag{\Delta}^{\ell\lambda}_k : k\ell\lambda$ holds by inductive hypothesis by setting $k = k\ell$.
  The case for \textsc{ParR} is analogous to the case for \textsc{ParL}.

  Finally, the \textsc{Congr} rule is simply resolved by induction, since its trivial to show that the congruence relation does not change the barbs expressed by a distribution.
\end{proof}


==> Sections/prop.tex <==
A consequence of~\autoref{thm:propertyA} is that $\sim_{cs}$ is not decomposable, similarly to other proposals addressing the limitations of probabilistic bisimilarity~\cite{fengtoward2015-1,dengbisimulations2018}.
\begin{corollary}
	cs-bisimilarity is not a decomposable relation.
\end{corollary}
\begin{proofsketch}
	Take $\Delta = \sconf{\ketbra{0}, c!q}\psum{{1}/{2}}\sconf{\ketbra{1}, c!q}$ and  
	$\Theta = \sconf{\ketbra{+}, c!q}\psum{{1}/{2}}\sconf{\ketbra{-}, c!q}$.
	Notice that $\Delta \sim_{cs} \Theta$ by~\autoref{thm:propertyA}.
	Then, for $\sim_{cs}$ to be decomposable, $\Theta$ should be equal to $\Theta_1\psum{{1}/{2}}\Theta_2$ for some $\Theta_1 \sim_{cs} \sconf{\ketbra{0}, c!q}$.
	But since $\Theta_1$ can only be either $\sconf{\ketbra{+}, c!q}$, $\sconf{\ketbra{-}, c!q}$ or a combination of them, $\Theta_1 \not\sim_{cs} \sconf{\ketbra{0}, c!q}$ as they send observably different quantum values.
\end{proofsketch}

We now investigate our cs-bisimilarity.
We first recover two defining properties of~\cite{dengopen2012}, 
namely that $\sim_{cs}$ is closed for superoperator application on qubits not appearing in the processes,
and that the state of such qubits is required to match in bisimilar distributions.
Then we show that discarded qubits can be ``traced out'' from the quantum state without affecting bisimilarity.
Finally, we discuss up-to techniques for proving constrained bisimilarity.

We start by recovering trace-identity and closure over superoperator application.
\begin{restatable}{proposition}{thmchinese}\label{thm:qccs}
	Let $\singleton{\conf{\rho, P, \nil}} \sim_{cs} \singleton{\conf{\sigma, Q, \nil}}$,
	then
	\begin{enumerate}
		\item $\singleton{\conf{\sop[\tilde{q}]{E}{\rho}, P, \nil}} \sim_{cs} \singleton{\conf{\sop[\tilde{q}]{E}{\sigma}, Q, \nil}}$, for any $\mathcal{E}_{\tilde{q}}$ and $\tilde{q}$ not in $\tilde{\Sigma}_P$;
		\item $\tr_{\Sigma_P}(\rho) = \tr_{\Sigma_P}(\sigma)$.
	\end{enumerate}
\end{restatable}
\begin{proofsketch}
	For the first point, take any superoperator $\mathcal{E}_{\tilde{q}}$, then there is a context that performs such transformation, so a context-closed relation is necessarily superoperator-closed. 
	For the second one, we proceed by contradiction: if the reduced density operators of two configurations are different, then we can build a context which measures such qubits obtaining a different distribution of outcomes and thus distinguishing the configurations via fresh barbs. 
\end{proofsketch}
Note that this is a useful result for disproving bisimilarity, as e.g., distributions with different partial trace are immediately deemed distinguishable.

A result that helps instead in proving bisimilarity is that the state of discarded qubits can be ignored.
In order to prove this in general, we extend the partial trace as follows.
\begin{definition}
	The partial trace $\ptrace{q}{\conf{\rho, P}}$ over $\tilde{q}$ of a configuration 
	is defined as $\conf{\ptrace{q}{\rho}, P'}$ if $P \equiv P' \parallel \nil_{\tilde{q}}$. 
	We let $\ptrace{q}{\bot} = \bot$, and define the partial trace of distributions by linearity.
\end{definition}
Intuitively, we remove the discarded qubits \emph{together with} the discard processes.
Note that such an operation is defined only on distributions of configurations that discard the same qubits.

\begin{restatable}{proposition}{bisimilaritydiscarded}\label{thm:discarded}
	Let $\Delta, \Theta$ be distributions such that $\ptrace{q}{\Delta}$ and $\ptrace{q}{\Theta}$ are well-defined for a given $\tilde{q}$. If $\ptrace{q}{\Delta} \sim_{cs} \ptrace{q}{\Theta}$ then $\Delta \sim_{cs} \Theta$.
\end{restatable}
\begin{proofsketch}
	We show, by induction on $\longsquiggly_\pi$, that the semantics of $\mathcal{C}$ and of $\ptrace{q}{\mathcal{C}}$ are equivalent, and since the partial trace does not affect barbs, the desired property follows.
\end{proofsketch}
Note that, even if this property is given for the process $\nil_{\tilde{q}}$, we can apply it to any ``discard-like'' process thanks to the linearity of $\sim_{cs}$, i.e.\ to any process bisimilar to $\nil_{\tilde q}$.

The capacity to ignore discarded qubit is useful in a lot of proofs, as for the example below proving that Alice cannot communicate with Bob in~\autoref{ex:light}.
\begin{example}
	The two distributions below are bisimilar
	\begin{gather*}
		\Delta = \singleton{\conf{\dket{\Phi^+}, \meas[M_{01}]{q_1}{x}.\nil_{q_1}}} \text{ and }
		\Theta = \singleton{\conf{\dket{\Phi^+}, \meas[M_\pm]{q_1}{x}.\nil_{q_1}}}
	\end{gather*}
	Taken any $B[\blank]$, they evolve in $B[\Delta']$ with
	$\Delta' = \Big(\singleton{\conf{\dket{00}, c!q_1}} \psum{{1}/{2}} \singleton{\conf{\dket{11}, c!q_1}}\Big)  \parallel \nil_{q_2}$ and $O[\Theta']$ with
	$\Theta' = \Big(\singleton{\conf{\dket{++}, c!q_1}}  \psum{{1}/{2}} \singleton{\conf{\dket{--}, c!q_1}}\Big) \parallel \nil_{q_2}$.
	
	Finally, note that $\tr_{q_2}(\Delta') \sim_{cs} \tr_{q_2}(\Theta')$ holds because $\tr_{q_2}(\Delta') = \singleton{\conf{\dket{0}, c!q_1}} \psum{{1}/{2}} \singleton{\conf{\dket{1}, c!q_1}}$ and $\tr_{q_2}(\Theta') = \singleton{\conf{\dket{+}, c!q_1}}  \psum{{1}/{2}} \singleton{\conf{\dket{-}, c!q_1}}$, and the two are equated by~\autoref{thm:propertyA}.
\end{example}



==> Sections/real-world.tex <==

\red{\textbf{Con week scheduler vince Alice, con strong vince Bob -- forse servono simulations}}

We present now a more complex example, namely the Quantum Coin Flipping (QCF) protocol. 
Suppose Alice and Bob do not trust each other, and want to randomly select a winner between them.
\cite{bb84} propose a protocol in which Alice chooses either the $01$ or $\pm$ basis at random, then generates a sequence of random bits and encodes them into a sequence of qubits in the selected basis (the first element of the basis stands for bit $0$, the second for $1$).
The qubits are then sent to Bob, who 
measures each of them in a random basis ($01$ or $\pm$). Finally, Bob tries to guess the basis chosen by Alice: Bob wins if the guess is correct. 

Bob has no way to find Alice's basis from the received qubits, so the guess will be correct or wrong with equal probability. 
Alice could cheat, lying about their basis. 
To protect Bob, at the end of the protocol, Alice must reveal their basis and the original bit sequence.
Bob then compares the original sequence with the previously stored outcomes of the measurements.
For qubits where Alice's basis coincides with Bob's one, the outcomes must 
coincide with the original bit sequence.

Hereafter, we let $x_i$ be the $i$-th bit of the integer $x$, and resort to some minor extensions of lqCCS\@
\begin{itemize}
\item $\conf{\rho, RandBit(x).P}$ evolves as $\overline{\conf{\rho, P[0/x]}} \psum{{1}/{2}} \overline{\conf{\rho, P[1/x]}}$, and could be implemented with an additional qubit.
\item We assume a mapping $\beta$ from bit to bases with $\beta(0)$ and $\beta(1)$ the $01$ and $\pm$ basis. 
\item We assume a polyadic extension of lqCCS type system and semantics where $c!\tilde{v}$ and $c?\tilde{x}$ allow substituting tuples of values $\tilde{v} = v_1, \ldots ,v_n$ for variables $\tilde{x} = x_1, \ldots ,x_n$.
\end{itemize} 

We formalize QCF as follows, where $n$ is the number of qubits, and the outcome is sent on $a$ and $b$ ($1$ if Bob wins and $0$ otherwise).
We use $b =_{int} b'$ for comparing digits, defined as $(1 - b)(1 - b') + bb'$.
\begin{align*}
  \proc{Alice}       & = Rand(\text{secretvalue}).\proc{Alice}_{\beta(\text{secretvalue})}                                                               \\
  \proc{Alice}_{01}  & = \unitary{H}{\tilde{q}}.M_{01}(\tilde{q} \rhd w).(
	\mathit{AtoB}!\tilde{q} \parallel
	\mathit{guess}?g.(a!(g =_{int} 0)
	 \parallel \mathit{secret}!0 \parallel \mathit{witness}!w
	))                                                                                                       \\
	\proc{Alice}_{\pm} & = I(\tilde{q}).M_\pm(\tilde{q} \rhd w).(
	\mathit{AtoB}!\tilde{q} \parallel
	\mathit{guess}?g.(a!(g =_{int} 1)
	\parallel \mathit{secret}!1 \parallel \mathit{witness}!w
	))                                                                                                       \\
	\proc{Bob}         & = \mathit{AtoB}?\tilde{z}.\Big(
	\Big(\Big(\bigparallel\nolimits_{i = 1}^n \proc{Server}_i \Big) \parallel \proc{Bob}' \Big) \setminus \{\mathit{base}_i\}_{i = 1}^n \setminus \{\text{bit}_i\}_{i = 1}^n
	\Big)                                                                                                       \\
	\proc{Bob}'        & = \mathit{base}_1?b_1\ldots \mathit{base}_n?b_n.
	\mathit{bit}_1?x_1\ldots\mathit{bit}_n?x_n.
	Rand(g).(\mathit{guess}!g \parallel \proc{Bob}'')                                                                  \\
	\proc{Bob}''       & =  \mathit{secret}?g'.\mathit{witness}?w.\Big(
	b!(g =_{int} g') \parallel
	\Big(\bigparallel\nolimits_{i = 1}^n
	\ite{(b_i = g' \land x_i \neq w_i}{\mathit{cheat}!0}{\nil}
	\Big)\Big)                                                                                                       \\
	\proc{Server}_i    & = Rand(b).M_{\beta(b)}(z_i \rhd x).(\mathit{base}_i!b \parallel \mathit{bit}_i!x \parallel \nil_{z_i}) \\
	\proc{QCF} 				& = (\proc{Alice} \parallel \proc{Bob}) \setminus \{\mathit{AtoB, guess, secret, witness}\} 									
\end{align*}
Thanks to cs-bisimilarity, we can analyse three properties of QCF, namely that the outcome is fair, that Bob cannot cheat, and neither Alice can. As reported by~\cite{bb84}, the first two properties hold, but an attack exists allowing Alice to decide the outcome of the protocol.
\paragraph{Fairness}
We show that $\conf{\ketbra{0^n}, \proc{QCF}} \sim_{cs} \conf{\ketbra{0^n}, \proc{FairCoin}}$, with $\proc{FairCoin}$ defined as $\tau^{4n + 5}.Rand(x).(a!x \parallel \tau.\tau.b!x \parallel \nil_{\tilde{q}})$.
As before, it suffices to consider the empty context, and we show the evolution of the protocol for $n = 1$, as the other cases follow the same pattern.
\[
\conf{\ketbra{0}, \proc{QCF}}
\longsquiggly_\diamond \left(\overline{\conf{\ketbra{0}, \proc{Alice}_{01}\parallel \proc{Bob}}} \psum{\frac{1}{2}}
\overline{\conf{\ketbra{0}, \proc{Alice}_{\pm}\parallel \proc{Bob}}}\right) \setminus C
\]
where $C = \{\mathit{AtoB, guess, secret, witness}\}$. We will focus just on the execution of $Alice_{01}$, as the other one is symmetrical. The first actions of Alice are to prepare the qubit at random and send it to Bob. The latter will then measure it in a random basis and record the result. Formally
\begin{align*}
& \conf{\ketbra{0}, \proc{Alice}_{01}\parallel \proc{Bob}}\\
& \longsquiggly_\diamond^3
\sum\nolimits_{j \in \{0, 1\}} \distelem{\frac{1}{2}}{\overline{\conf{\ketbra{j}, \proc{Alice}_{01}'[j/w] \parallel  \proc{Bob}' \parallel \proc{Server}}}}		\\
& \longsquiggly_\diamond^2
\quad \distelem{\frac{1}{2}}{\left(\sum\nolimits_{j \in \{0, 1\}} \distelem{\frac{1}{2}}{\overline{\conf{\ketbra{j}, \proc{Alice}_{01}'[j/w] \parallel \proc{Bob}' \parallel (\mathit{base}!0 \parallel \mathit{bit}!j \parallel \nil_{q}) }}}\right)} \\
& \qquad \ +\distelem{\frac{1}{2}}{\left(\sum\nolimits_{j \in \{0, 1\}} \distelem{\frac{1}{2}}{\overline{\conf{H\ketbra{j}H, \proc{Alice}_{01}'[j/w] \parallel \proc{Bob}' \parallel (\mathit{base}!1 \parallel \mathit{bit}!j \parallel \nil_{q}) }}}\right)} 
\end{align*}																							
where $\proc{Alice}_{01}' = \mathit{guess}?g.(a!(g =_{int} 0) \parallel \mathit{secret}!0 \parallel \mathit{witness}!w)$.
After the measurement (and after synchronising with the server processes) Bob send their random guess of the secret basis to Alice, who reveals the correct one.
Bob checks the consistency of Alice response, and if the protocol is executed correctly the two parties will agree on the outcome: either $0$ or $1$ with equal probability.
\begin{align*}
&
\quad \distelem{\frac{1}{2}}{\left(\sum\nolimits_{j, k \in \{0, 1\}}\distelem{\frac{1}{4}}{\overline{\conf{\ketbra{j},\nil_{q} \parallel \proc{Alice}_{01}'[j/w] \parallel \mathit{guess}!k \parallel \proc{Bob}''[0/b][j/x][k/g] }}}\right)} \\
& +\distelem{\frac{1}{2}}{\left(\sum\nolimits_{j, k \in \{0, 1\}}\distelem{\frac{1}{4}}{\overline{\conf{H\ketbra{j}H,\nil_{q} \parallel \proc{Alice}_{01}'[j/w] \parallel \mathit{guess}!k \parallel \proc{Bob}''[1/b][j/x][k/g] }}}\right)} \\
& \longsquiggly_\diamond^3
{\left(\sum\nolimits_{j, k \in \{0, 1\}} \distelem{\frac{1}{4}}{\overline{\conf{\ketbra{j},\nil_{q} \parallel a!k \parallel b!k }}}\right)} 
\ \psum{\frac{1}{2}} \ {\left(\sum\nolimits_{j, k \in \{0, 1\}} \distelem{\frac{1}{4}}{\overline{\conf{H\ketbra{j}H,\nil_{q} \parallel a!k \parallel b!k }}}\right)} 
\end{align*}
 It is easy to see that in this last step $\proc{QCF}$ expresses the barbs $\downarrow a$ and $\downarrow b$, sending the same values as the specification $\proc{FairCoin}$, and the two are indeed bisimilar.

\paragraph{Dishonest Bob}
In order to cheat, Bob needs to discover
Alice's secret from the sent qubits alone. 
This is impossible, because \autoref{thm:propertyA} deems the initial prefixes of $\proc{Alice}_{01}$ and $\proc{Alice}_\pm$ bisimilar.
\[
	\proc{A}_{01} = \sum\nolimits_{j = 0}^{2^n-1} \distelem{\frac{1}{2^n}}{\conf{\ketbra{j}, AtoB!\tilde{q}}} \quad \sim_{cs}  \quad \sum\nolimits_{j = 0}^{2^n-1} \distelem{\frac{1}{2^n}}{\conf{H^{\otimes n}\ketbra{j}H^{\otimes n}, AtoB!\tilde{q}}} = \proc{A}_\pm
\]
Note that $A_{01} \not\sim_s A_{\pm}$, as shown in~\autoref{ex:broken-nondet}.
	Traditional probabilistic bisimilarity à la~\cite{hennessyexploring2012} 
	fails in analysing Quantum Coin Flipping and similar protocols.

\paragraph{Dishonest Alice}

Interestingly, Alice can cheat by using additional qubits entangled with the ones they send to Bob. 
By measuring their entangled qubits in Bob's chosen basis, Alice forges a fake witness for deceiving Bob (in the process, Alice wins and $0$ is sent on $a$ and $b$). 
We call this attacker 
Alison, and show that $\conf{\ketbra{0^{2n}}, (\proc{Alison} \parallel \proc{Bob}) \setminus C} \sim_{cs} \conf{\ketbra{0^{2n}}, \proc{UnfairCoin}}$.
\begin{align*}
	\proc{Alison}  & = Set_{\Phi^+}(q_1, q_1')\ldots Set_{\Phi^+}(q_n, q_n').\left(
	\mathit{AtoB}!\tilde{q} \parallel \proc{Alison}'
	\right)                                                                                                                                                 \\
	\proc{Alison}' & = \mathit{guess}?g.(a!0 \parallel \mathit{secret}!(1 - g) \parallel M_{\beta(1-g)}(q' \rhd x').(\mathit{witness}!x' \parallel \nil_{\tilde{q'}})) \\
	\proc{UnfairCoin}     & = \tau^{5n + 3}.(a!0 \parallel \tau.\tau.\tau.b!0 \parallel \nil_{\tilde{q}} \parallel \nil_{\tilde{q'}})
\end{align*}
The $\proc{UnfairCoin}$ specification always selects Alison as the winner, and never expresses the $\downarrow_{cheat}$ barb. In other words, $(\proc{Alison} \parallel \proc{Bob}) \setminus C \sim_{cs} \proc{UnfairCoin}$ means that Alison is always capable of tricking Bob without being discovered. 

The behaviour of Bob is identical to the previous case.
Indeed, the reduced density operator of the qubits sent by Alison is indistinguishable from the one of the honest Alice. 
But after receiving Bob's guess, Alison can measure their own qubits, which have decayed as the ones of Bob. 
In this way, her fake witness $w'$ will always be correct, as we show for the case $n = 1$
\begin{align*}
  & \conf{\ketbra{00}, (\proc{Alison} \parallel \proc{Bob}) \setminus C}  \\
& \longsquiggly_\diamond^{11}
{\left(\sum\nolimits_{j \in \{0, 1\}} \distelem{\frac{1}{2}}{\overline{\conf{\ketbra{jj},\nil_{q} \parallel a!0 \parallel b!0 }}}\right)} 
\ \psum{\frac{1}{2}} \ {\left(\sum\nolimits_{j \in \{+, -\}} \distelem{\frac{1}{2}}{\overline{\conf{\ketbra{jj},\nil_{q} \parallel a!0 \parallel b!0 }}}\right)}
\end{align*}


==> Sections/rw.tex <==

As a result of our saturated approach, entangled pairs are correctly distinguished from separable states with the same partial trace (see the fourth row of the same table).
\begin{example}\label{ex:entanglement}
	The processes in the fourth row of~\autoref{tab:examples} are distinguished by the context $B[\blank] = [\blank] \parallel c?x.c?y.\meas{x, y}{z}.(\ite{z = (01)_2}{d!0}{\nil} \parallel \nil_{x, y})$,
	because it will eventually exhibit the barb $d$ if the state decays in $\ket{01}$ (which is only possible for $\frac{1}{4} I$).
\end{example}

Finally, notice that saturated bisimilarity equates the discard process $\nil_{q_1,q_2}$ with both $\nil_{q_2,q_1}$ and $c?x.(c!q_1 \parallel c!q_2 \parallel c!x) \setminus c$.
To prove that, it suffices to give the relation associating $\Delta$ with $\Delta[\sfrac{P}{Q}]$ for any choice of $P$ and $Q$ among the processes above.
This is clearly a bisimulation, once closed for contexts and congruence: for any context $B[\blank]$, if $B[P] \rightarrow \Delta$ then $B[Q] \rightarrow \Delta[\sfrac{P}{Q}]$.


We focus on the quantum process calculi most similar to our proposal,
as well as likely the better established and developed, namely QPAlg~\cite{lalireproces2004,lalirerelations2006}, CQP~\cite{gaycommunicating2005,gaytypes2006,davidsonformal2012}, and qCCS~\cite{fengprobabilistic2007,yingalgebra2009,fengbisimulation2012,fengsymbolic2014,dengopen2012,fengtoward2015-1,dengbisimulations2018}\@.
When comparing the proposed behavioural equivalences, we abstract from the ``classical'' details 
and focus on the quantum-related features,
restricting ourselves to the strong version of the bisimulations.
A first difference with lqCCS is that they are mostly based on labelled bisimilarities.
\autoref{tab:examples} summarizes distinctive prototypical processes (in the lqCCS syntax) deemed bisimilar or not according to different approaches.

One of the discrepancies is the visibility of qubits that are neither sent nor discarded.
The first three lines contain processes whose bisimilarity depends on the assumption about the visibility of these unsent qubits.
Our linear type system makes the former assumptions irrelevant.
In the fourth line, the processes send pairs of qubits with the same partial trace if taken separately, even if a pair is entangled and the other is not.
The fifth line compares processes where the state of the sent qubits is represented by the same density operator,
whose bisimilarity is implied by~\autoref{thm:propertyA}.
Finally, the sixth line compares two processes where a qubit is sent non-deterministically over two channels:
for each channel, the state of the sent qubits is represented by the same density operator, but if the chosen channel depends on the outcome of the measurement the two processes can be distinguished.
	Bisimilarities that do not distinguish these two processes cannot satisfy~\autoref{thm:nondetVSite}.

\subsection*{QPAlg}
The Quantum Process Algebra (QPAlg) is an extension of synchronous value-passing
CCS with primitives for unitary transformations and measurements.
As common, quantum operations are silent, and quantum communication updates quantum variables.
They propose a probabilistic branching
bisimilarity, adapted for stateful computations by requiring
bisimilar processes to send the same quantum state, defined as the partial trace of the global quantum
state.
However, this bisimilarity is coarser than prescribed by the theory when states are entangled~\cite{davidsonformal2012}.
\begin{example}\label{ex:qpalg}
	The processes in the fourth line of~\autoref{tab:examples} are bisimilar in QPAlg, as they send pairs of qubits with the same partial trace
	($tr_{q_0}(\Phi^+) = tr_{q_1}(\Phi^+) = tr_{q_0}(\frac{1}{4}I) = tr_{q_1}(\frac{1}{4}I) = \frac{1}{2}I$).
	Such processes are not bisimilar according to $\sim_{cs}$, as the context of~\autoref{ex:entanglement} discriminates the two.
\end{example}
Finally, behaviourally equivalent processes are not required to behave similarly on unsent qubits,
e.g.\ $H(q).\nil$ and $X(q).\nil$ of the first line of~\autoref{tab:examples}.
In lqCCS, the above processes are not legal, but a similar result holds for $H(q).\nil_{q}$ and $X(q).\nil_{q}$.

\subsection*{CQP}

The calculus of Communicating Quantum Processes (CQP) is inspired by the $\pi$-calculus and it is enriched with qubits declarations (that extend the quantum state) and quantum transformations,
but without guards or match operators, thus lacking the form of classical control used in lqCCS\@.
They introduce an affine type system prescribing that every qubit is sent at most once.
CQP comes with a reduction semantics~\cite{gaycommunicating2005,gaytypes2006} and a labelled one~\cite{davidsonformal2012}, both based on pure quantum states.
Davidson proposes mixed configurations, i.e.\ configurations where a single process is paired with a probability distribution of classical and quantum states.
Mixed configurations represent non-observable probabilities due to measurements whose result is not communicated yet, and they are treated as a single state by the semantics.
Our proposal generalizes CQP mixed configurations to distributions of configurations with possibly different processes.
This is necessary for extending the approach to processes with boolean guards.

A branching bisimilarity is defined for the labelled semantics of CQP\@.
To avoid the problem of QPAlg with entangled states, bisimilarity requires that the reduced state obtained by collecting \emph{all} the sent qubits coincide.
Moreover, mixed configurations allow relating processes sending indistinguishable quantum states.
The resulting bisimilarity is a congruence for parallel
composition and is capable of equating interesting cases such as the one of the fifth line of~\autoref{tab:examples}.
\begin{example}
  Consider $\conf{\dket{+}, \meas[M_{01}]{q}{x}.c!q}$ and $\conf{\dket{0}, \meas[M_{\pm}]{q}{x}.c!q}$.
	Even though they end up in different quantum states, the two configurations above are bisimilar according to CQP, because they send on channel $c$ qubits with the same partial trace.
	Our proposed bisimilarity replicates this result by resorting to contexts with constrained non-determinism (see~\autoref{ex:zopm}). 
	Indeed, a context receiving the qubit cannot behave differently depending on its state if not through measurement, and when measured, the states of the two qubits coincide.
\end{example}
Our cs-bisimilarity extends the one of CQP in a context-based fashion over standard distributions.
CQP behaves as QPAlg with respect to unsent qubits (see the first line of~\autoref{tab:examples}).

\subsection*{qCCS}

Our process calculus takes its most direct inspiration from qCCS, a synchronous
CCS-style calculus with superoperators and measurements where
syntactic restrictions guarantee each qubit is sent at most once.
A feature of qCCS is the support for recursive processes, which we postpone to future work.
Two different labelled bisimilarities are proposed for qCCS\@: the first is based on standard probabilistic bisimulations; the second one relies on transition consistency and subdistributions.

The probabilistic bisimilarity~\cite{fengprobabilistic2007,fengbisimulation2012} (denoted by $\sim_{p}$ in \autoref{tab:examples}) requires bisimilar processes to send the same names on the same channels and to produce the same quantum state of qubits that are not owned any more.
In addition, bisimulations must be closed under applications of trace-preserving superoperators on not-owned qubits.
Therefore, the 
processes of the first line of~\autoref{tab:examples} are distinguished.
We recover this assumption by sending the qubits (see the third line).

Moreover, \autoref{thm:qccs} shows that cd-bisimilarity replicates the $\sim_p$ requirements over superoperators and not owned qubits.
The probabilistic bisimilarity of qCCS is proved to be a congruence with respect to parallel composition.
Further extensions are the (weak) open bisimilarity proposed in~\cite{dengopen2012}, proven to be a weak barbed congruence, and a symbolic version of the bisimilarity in~\cite{fengsymbolic2014},
that relieves from considering all the (universally quantified) quantum states of a configuration when verifying bisimilarity.

Configurations like the ones of the fifth line of~\autoref{tab:examples} are not bisimilar for $\sim_p$, even though they are indistinguishable according to quantum theory.
This discrepancy was signalled in~\cite{kubotaapplicationnoyear} and lead to a new proposal called distribution bisimilarity~\cite{fengtoward2015-1,dengbisimulations2018} (denoted by $\sim_{d}$ in \autoref{tab:examples}), which is directly defined on distributions and is based on transition consistency.
A distribution is called transition consistent if any configuration in its support has exactly the same set of enabled visible actions.
In addition to closure with respect to superoperator application, bisimilar distributions are required to be such that: $(i)$ the weighted sums of the state of not owned qubits in the support coincide; $(ii)$ the possible transitions of one transition consistent distribution
are matched by the other one, and; $(iii)$ if the distributions are not transition consistent, then they must be decomposable in bisimilar transition consistent distributions.
On the one hand, considering distributions as a whole when comparing the quantum states equates processes like the ones of the fifth line of~\autoref{tab:examples}.
On the other hand, transition consistent decompositions recover a weakened version of decomposability, avoiding equating distributions that cannot evolve because the processes in the supports enable different actions only.

The use of transition consistency in $\sim_d$ implicitly constrains non-determinism.
In the last line of~\autoref{tab:examples}, we compare such constraints with the ones we impose on lqCCS\@.
While our $\sim_{cs}$ is capable of distinguishing the two processes, $\sim_d$ cannot.
In fact, the lifting of the \emph{labelled} semantics of qCCS forbids processes from replicating the moves of their refinements (as lqCCS does).
\begin{example}
	Consider the pair of processes of the last line of~\autoref{tab:examples}. They reduce to
	\begin{gather*}
		\Delta = \overline{\conf{\dket{0}, c!q + d!q}} \psum{1/2} \overline{\conf{\dket{1}, c!q + d!q}} \quad
		\Theta = \overline{\conf{\dket{+}, c!q + d!q}} \psum{1/2} \overline{\conf{\dket{-}, c!q + d!q}}
	\end{gather*}
	We show in~\autoref{ex:non-detproc2} that $\Delta \not\sim_{cs} \Theta$, as $\Delta$ can choose to send the qubit over $c$ only when it is set to $\kz$, while $\Theta$ cannot.
	In the distribution bisimulation of~\cite{fengtoward2015-1}, instead, only the moves that choose the same channel in all the configurations of the support are considered, deeming the two distributions bisimilar.
  This means that $\meas[M_{01}]{q}{x}. (c!q + d!q)$ cannot use the value of $x$ to choose the channel over which to send, as it would be expected, and thus that the constraints over non-determinism are arguably too strong in~\cite{fengtoward2015-1}.
\end{example}

Finally, \cite{fengtoward2015-1} acknowledge that \emph{weak} distribution bisimilarity is not a congruence.
Its strong version is not a congruence either: take $\Delta \sim_{d} \Theta$ and $B[\blank]$ of~\autoref{ex:broken-nondet}, it is easy to show that $B[\Delta] \not\sim_{d} B[\Theta]$.
The same also holds for $\sim_{cs}$, which is a congruence with respect to observers but not to parallel composition.
We believe that $\sim_{d}$ actually verifies the indistinguishability property over deterministic processes of~\autoref{thm:propertyA}, 
and
$B[\Delta] \not\sim_{d} B[\Theta]$ shows that the result cannot be extended to general processes.
On a similar note, 
$\sim_{d}$ does not preserve the expressiveness 
of non-deterministic choices based on classical information stated in~\autoref{thm:nondetVSite}.






